Deep Reinforcement Learning for Efficient and Fair Allocation of Health Care Resources

Scarcity of health care resources could result in the unavoidable consequence of rationing. For example, ventilators are often limited in supply, especially during public health emergencies or in resource-constrained health care settings, such as amid the pandemic of COVID-19. Currently, there is no universally accepted standard for health care resource allocation protocols, resulting in different governments prioritizing patients based on various criteria and heuristic-based protocols. In this study, we investigate the use of reinforcement learning for critical care resource allocation policy optimization to fairly and effectively ration resources. We propose a transformer-based deep Q-network to integrate the disease progression of individual patients and the interaction effects among patients during the critical care resource allocation. We aim to improve both fairness of allocation and overall patient outcomes. Our experiments demonstrate that our method significantly reduces excess deaths and achieves a more equitable distribution under different levels of ventilator shortage, when compared to existing severity-based and comorbidity-based methods in use by different governments. Our source code is included in the supplement and will be released on Github upon publication.

==> Sections/checklist.tex <==
\section{Reproducibility Checklist}
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced \textit{YES}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results \textit{YES}
    \item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper \textit{YES}
\end{itemize}

\subsection{Theoretical Contributions}
\textbf{Does this paper make theoretical contributions?} \textit{No, The topic we are addressing is NP-hard in nature. While the theoretical proof could be interesting, it falls outside the primary objective of this study. Instead, we offer strong empirical results as an alternative.}

If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. 
    \item All novel claims are stated formally (e.g., in theorem statements).
    \item Proofs of all novel claims are included.
    \item Proof sketches or intuitions are given for complex and/or novel results. 
    \item Appropriate citations to theoretical tools used are given.
    \item All theoretical claims are demonstrated empirically to hold.
    \item All experimental code used to eliminate or disprove claims is included. 
\end{itemize}

\subsection{Dataset Utilization}
\textbf{Does this paper rely on one or more datasets?} \textit{yes}

If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets \textit{yes}
    \item All novel datasets introduced in this paper are included in a data appendix. \textit{no}, we will open-source the de-identified dataset upon acceptance. The dataset contains personal health information and cannot be shared as an appendix which violates the HIPAA regulation.
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textit{yes}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \textit{NA}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \textit{NA}
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \textit{NA}
\end{itemize}

\subsection{Computational Experiments}
\textbf{Does this paper include computational experiments? (yes/no)} \textit{yes}

If yes, please complete the list below.
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. \textit{yes}
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. \textit{yes}
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textit{yes}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from \textit{yes}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \textit{yes}
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \textit{yes}
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \textit{yes}
    \item This paper states the number of algorithm runs used to compute each reported result. \textit{yes}
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \textit{yes}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \textit{yes}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \textit{yes}
    \item This paper states the number and range of values tried per (hyper-)parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \textit{yes}
\end{itemize}



==> tables/table2.tex <==
% \begin{table}[t]
% \centering
% \caption{Impact of triage protocols on survival, fairness, and allocation rates with limited ventilators (B = 40) corresponding to about 50\% scarcity. TDDQN and TDDQN-fair are without and with fairness rewards, respectively. Fairness metric is demographic parity ratio (DPR, the ratio between the smallest and the largest allocation rate across patient groups,  100\% indicating non-discriminative). Standard deviations are from 10 experiments with different seeds. We bold the ethnoracial group results with the highest survival rate, DPR, and overall allocation rates. We underline the metrics that fall within one standard deviation of the best result.} % The initial four protocols serve as baseline protocols. 
% \label{tab:tab2}
% \vskip 0.15in
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}l|l|l|lllll@{}}
% \toprule
%                   & \textbf{Performance} & \textbf{Fairness} & \multicolumn{5}{l}{\textbf{Allocation Rates}}                            \\ \cmidrule(l){2-8} 
%                   & Survival, \%            & DPR, \%           & Overall, \%  & Asian, \%    & Black, \%    & Hispanic, \% & White, \%    \\ \midrule
% \textbf{Lottery}    & 75.17 ± 0.45          & \textbf{96.89 ± 1.55} & 75.60 ± 0.28          & 74.95 ± 1.81 & 75.65 ± 1.10 & 76.08 ± 0.90 & 75.68 ± 0.33 \\
% \textbf{Youngest} & 77.24 ± 0.07         & 86.39 ± 0.27      & 75.65 ± 0.09 & 75.59 ± 0.50 & 81.73 ± 0.31 & 84.44 ± 0.30 & 72.94 ± 0.12 \\
% \textbf{SOFA}     & 80.88 ± 0.32         & 92.37 ± 1.01      & 77.92 ± 0.25 & 75.06 ± 1.44 & 73.58 ± 0.77 & 78.66 ± 1.24 & 79.10 ± 0.45 \\
% \textbf{DT}       & 81.99 ± 0.14         & 90.68 ± 0.95      & 78.34 ± 0.20 & 77.91 ± 1.48 & 74.33 ± 0.66 & 81.96 ± 0.56 & 78.81 ± 0.34 \\ 
% \textbf{MP}       & 81.99 ± 0.14         & 90.68 ± 0.95      & 78.34 ± 0.20 & 77.91 ± 1.48 & 74.33 ± 0.66 & 81.96 ± 0.56 & 78.81 ± 0.34 \\ \midrule
% \textbf{TxDDQN}    & 84.76 ± 0.24         & 86.91 ± 3.45      & \underline{81.80 ± 0.26} & 78.03 ± 0.99 & 72.48 ± 0.74 & 81.71 ± 0.44 & 84.45 ± 0.22 \\
% \textbf{TxDDQN-fair} & \textbf{85.41 ± 0.23} & \underline{95.24 ± 1.65}          & \textbf{81.90 ± 0.24} & 80.01 ± 1.79 & 79.95 ± 1.05 & 81.26 ± 1.24 & 82.80 ± 0.42 \\
% \textbf{TxDDQN-fair-off} & \textbf{85.41 ± 0.23} & \underline{95.24 ± 1.65}          & \textbf{81.90 ± 0.24} & 80.01 ± 1.79 & 79.95 ± 1.05 & 81.26 ± 1.24 & 82.80 ± 0.42 \\ \bottomrule
% \end{tabular}%
% }
% \vskip -0.1in
% \end{table}

\begin{table}[!t]
\setlength{\tabcolsep}{3pt}
\centering
\caption{Impact of triage protocols on survival, fairness, and allocation rates with limited ventilators (B = 40) corresponding to about 50\% scarcity. Fairness metric is demographic parity ratio (DPR, the ratio between the smallest and the largest allocation rate across patient groups,  100\% indicating non-discriminative). Standard deviations are from 10 experiments with different seeds. We bold the protocols with the highest survival rate, DPR, and overall allocation rates. We underline the protocols that fall within one standard deviation of the best result.}
\label{tab:tab2}
\vskip 0.15in
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|l|l|lllll@{}}
\toprule
                  & \textbf{Survival} & \textbf{Fairness} & \multicolumn{5}{l}{\textbf{Allocation Rates}}                            \\ \cmidrule(l){2-8} 
                  & Survival, \%            & DPR, \%           & Overall, \%  & Asian, \%    & Black, \%    & Hispanic, \% & White, \%    \\ \midrule
\textbf{Lottery}    & 75.17 \textpm \scriptsize{0.45} & \textbf{96.89 \textpm \scriptsize{1.55}} & 75.60 \textpm \scriptsize{0.28} & 74.95 \textpm \scriptsize{1.81} & 75.65 \textpm \scriptsize{1.10} & 76.08 \textpm \scriptsize{0.90} & 75.68 \textpm \scriptsize{0.33} \\
\textbf{Youngest} & 77.24 \textpm \scriptsize{0.07} & 86.39 \textpm \scriptsize{0.27} & 75.65 \textpm \scriptsize{0.09} & 75.59 \textpm \scriptsize{0.50} & 81.73 \textpm \scriptsize{0.31} & 84.44 \textpm \scriptsize{0.30} & 72.94 \textpm \scriptsize{0.12} \\
\textbf{SOFA}     & 80.88 \textpm \scriptsize{0.32} & 92.37 \textpm \scriptsize{1.01} & 77.92 \textpm \scriptsize{0.25} & 75.06 \textpm \scriptsize{1.44} & 73.58 \textpm \scriptsize{0.77} & 78.66 \textpm \scriptsize{1.24} & 79.10 \textpm \scriptsize{0.45} \\
\textbf{DT}       & 76.16 \textpm \scriptsize{0.01} & 94.35 \textpm \scriptsize{0.01} & 75.81 \textpm \scriptsize{0.01} & 79.59 \textpm \scriptsize{0.00} & 75.14 \textpm \scriptsize{0.01} & 77.34 \textpm \scriptsize{0.00} & 75.58 \textpm \scriptsize{0.00} \\ 
\textbf{MP}       & 81.99 \textpm \scriptsize{0.14} & 90.68 \textpm \scriptsize{0.95} & 78.34 \textpm \scriptsize{0.20} & 77.91 \textpm \scriptsize{1.48} & 74.33 \textpm \scriptsize{0.66} & 81.96 \textpm \scriptsize{0.56} & 78.81 \textpm \scriptsize{0.34} \\ \midrule
\textbf{TxDDQN}    & 84.76 \textpm \scriptsize{0.24} & 86.91 \textpm \scriptsize{3.45} & \underline{81.80 \textpm \scriptsize{0.26}} & 78.03 \textpm \scriptsize{0.99} & 72.48 \textpm \scriptsize{0.74} & 81.71 \textpm \scriptsize{0.44} & 84.45 \textpm \scriptsize{0.22} \\
\textbf{TxDDQN-fair-off} & \underline{85.29 \textpm \scriptsize{0.18}} & \underline{95.27 \textpm \scriptsize{1.42}} & \textbf{81.96 \textpm \scriptsize{0.15}} & 80.50 \textpm \scriptsize{2.23} & 80.07 \textpm \scriptsize{1.98} & 81.44 \textpm \scriptsize{1.05} & 82.70 \textpm \scriptsize{0.34} \\
\textbf{TxDDQN-fair} & \textbf{85.41 \textpm \scriptsize{0.23}} & \underline{95.24 \textpm \scriptsize{1.65}} & \underline{81.90 \textpm \scriptsize{0.24}} & 80.01 \textpm \scriptsize{1.79} & 79.95 \textpm \scriptsize{1.05} & 81.26 \textpm \scriptsize{1.24} & 82.80 \textpm \scriptsize{0.42} \\ \bottomrule
\end{tabular}%
}
\vskip -0.1in
\end{table}







